A Large Scale Benchmark and an Inclusion-Based Algorithm for Continuous Collision Detection

We introduce a large scale benchmark for continuous collision detection (CCD) algorithms, composed of queries manually constructed to highlight challenging degenerate cases and automatically generated using existing simulators to cover common cases. We use the benchmark to evaluate the accuracy, correctness, and efficiency of state-of-the-art continuous collision detection algorithms, both with and without minimal separation. We discover that, despite the widespread use of CCD algorithms, existing algorithms are either: (1) correct but impractically slow, (2) efficient but incorrect, introducing false negatives which will lead to interpenetration, or (3) correct but over conservative, reporting a large number of false positives which might lead to inaccuracies when integrated in a simulator. By combining the seminal interval root finding algorithm introduced by Snyder in 1992 with modern predicate design techniques, we propose a simple and efficient CCD algorithm. This algorithm is competitive with state of the art methods in terms of runtime while conservatively reporting the time of impact and allowing explicit trade off between runtime efficiency and number of false positives reported.

==> figures/old-proofs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\todo{this should say something like: all cases we consider are enough. The text here are different parts to get that}

For a bilinear patch defined by four segments $s_1$, $s_2$, $s_3$, $s_4$, if a line $l$ intersects it, then there is only one, or two, or infinite intersection points (infinite happens when: bilinear is flat while $l$ and bilinear are coplanar, or: $l$ and $s_i$ are colinear, or l is colinear with the ruler). 

\todo{merge here}

If a segment $S$ ( whose end points are $S_0$ and $S_1$, $S_0$ $\neq$ $S_1$ ) intersects with the tetrahedral $Tet$ defined by $s_1$, $s_2$, $s_3$, $s_4$, the volume of $Tet$ is not 0, and $S$ not intersects with any bilinear edges $s_i$. The segment has intersection with the bilinear ( the intersection is not a tangent point), if and only if one of the arguments below is true:\par
(1) if the segment $S$ is totally inside of $Tet$, and $\Phi(S_0)$ and $\Phi(S_1)$ has different signs;\par
(2) if $S$ has intersection with two facets $F_i$ and $F_j$ of $Tet$, and $\Phi(F_i)$, $\Phi(F_j)$ has different signs;\par
(3) if $S$ has intersection with one facet $F_i$, $S_0$ is inside $Tet$ and $S_1$ is outside, and $\Phi(F_i)$ and $\Phi(S_0)$ has different signs.\par
(4) if the line $l$ where the segment $S$ lies intersects two faces on the same side, find more than 1 roots using the root finder.\par
(5) phi(s0) or phi(s1) is 0.

\todo{merge with this}

Root finder:\todo{if the line intersect the different signs of facets, we don't need root finder}
When the segment has: \\
1. two intersection points with $F_i$,  $F_j$, but these two facets are on the same sides of the bilinear;\\
2. one intersection point with $F_i$, $S_0$ is inside of $Tet$, $\Phi(F_i)$ and $\Phi(S_0)$ has same signs, and the extension of $S$ intersects $F_j$,  $\Phi(F_i)$ is same with $\Phi(F_j)$.\\
3. zero intersection point, the segment totally inside $Tet$; $\Phi(S_0)$=$\Phi(S_1)$, the extension of $S$ intersects two same side facets of $Tet$,\\
then we need to use the root finder to find out if the segment has intersection with the bilinear (0 roots or 2 roots).
\end{lemma}
\begin{proof}
$\Phi$ is the implicit function of the bilinear patch (see Bridson). $\Phi$ is a quadratic function defined in a finite domain, and line function is a linear function, combine them together, the resulted function can have 0, 1, 2 or infinite roots. 

\todo{merge here}

from right to left: (1) (2) and (3) are proved in Bridson.proof of (4) sees below. from left to right: if the line expanded by the segment has only 1 intersection point with the bilinear, then it intersect facets with different signs of $\Phi$, (1) (2) and (3) can be obtained easily. if there are two intersection points between the line and the bilinear, then the line intersects the two facets on the same side.\todo{this is a bad proof} 
4. if a cube $Cb$ intersects the bilinear, then either the bilinear edges intersect the cube, or the cube edges intersects the bilinear.

\todo{merge here}

if these cases happen, since the function $\Phi$ is a quadratic function, if the sign of $\Phi$ of the segment end points are the same, there can be 0 or 2 intersections between the segment and the bilinear. \\\\
the root finder can be described like this:\\
$f=at^2+bt+c$, 0<=t<=1\\
if $f(0)$ or $f(1)==0$, true;\\
if $f(0)$, $f(1)$ has different signs, true;\\
if $f(0)$, $f(1)$ has same signs, if $a==0$, false;\\
if $0<=\bar{t}=-\frac{b}{2a}<=1$, $f(\bar{t})=\frac{4ac-b^2}{4a}$ has different sign with $f(0)$, then true;\\
\todo{we can use a table similar with Denish}

any other cases, false;\\
Caution: if $S$ has intersection with the $Tet$ surfaces, the region of t will not be [0,1] any more, instead, it will be $[\frac{n_1}{d_1},\frac{n_2}{d_2}]$, the root finder can be obtained similarly:\\\\
Set $a_1=d1^2*d2^2*a$,$b_1=d1^2*d2^2*b$,$c_1=d1^2*d2^2*c$, then $f(t_0)=a*d2^2*n1^2+b*d1*n1*d2^2+c*d1^2*d2^2$, $f(t_1)=a*d1^2*n2^2+b*d2*n2*d1^2+c*d1^2*d2^2$, $f(\bar{t})$ still has same sign with $\frac{4ac-b^2}{4a}$.\todo{delete this paragraph because we are not doing this}
\end{proof}
